A Multidimensional Elasticity Framework for Adaptive Data Analytics Management in the Computing Continuum

The increasing complexity of IoT applications and the continuous growth in data generated by connected devices have led to significant challenges in managing resources and meeting performance requirements in computing continuum architectures. Traditional cloud solutions struggle to handle the dynamic nature of these environments, where both infrastructure demands and data analytics requirements can fluctuate rapidly. As a result, there is a need for more adaptable and intelligent resource management solutions that can respond to these changes in real-time. This paper introduces a framework based on multi-dimensional elasticity, which enables the adaptive management of both infrastructure resources and data analytics requirements. The framework leverages an orchestrator capable of dynamically adjusting architecture resources such as CPU, memory, or bandwidth and modulating data analytics requirements, including coverage, sample, and freshness. The framework has been evaluated, demonstrating the impact of varying data analytics requirements on system performance and the orchestrator's effectiveness in maintaining a balanced and optimized system, ensuring efficient operation across edge and head nodes.

==> __3.Architecture.tex.v0 <==
\section{Adaptive Elasticity for Data Analytics in the CC} \label{Sec:architecture}



% The general dimensions of elasticity are subdivided into specific dimensions, which can be defined from two perspectives, at the operational level and at the application level as shown in Figure \ref{fig:elasticityDimensions}:
% \begin{itemize}
%     \item Computing Node Elasticity (operational level): refers to the dimensions that allow for adaptability of the computing nodes implemented in the infrastructure. The general dimensions covered are resources (to adjust CPU, memory, or energy consumption) and cost (to adjust the cost per use).
%     \item Analytic Elasticity (application level): refers to the dimensions that allow adapting the needs of the analytics proposed by the consumers. The general dimensions covered are quality (to adjust expected quality, expected response time, or frequency of the data) and cost (how much is willing to pay).
% \end{itemize}

%---------------%


Elasticity within the CC architecture is fundamental to enabling dynamic adaptation of both infrastructure resources and data analytics requirements. This elasticity spans multiple dimensions that impact both the operational efficiency and the performance of analytics applications. In this context, we propose a comprehensive framework for managing multi-dimensional elasticity in data analytics for the CC. These dimensions, illustrated in Fig.\ref{fig:elasticityDimensions}a, reflect the different factors that influence the adaptability of both computing resources and the data analytics themselves.


At the operational level, elasticity focuses on the efficient use of resources like CPU, memory, and energy, ensuring that these computing resources can be dynamically adjusted to changing workloads. This level also involves managing the cost associated with using infrastructure resources, particularly in environments where resource consumption is billed based on usage. At the application level, elasticity manages the specific requirements of data analytics, such as the quality of results, the frequency at which data is processed, and the timeliness of the analytics outcomes. These dimensions require careful balancing by the orchestrator to ensure that the infrastructure can meet performance expectations without exceeding resource or cost limitations. Furthermore, these dimensions are interrelated, since changes in one can affect others. Increasing the sample size to improve the quality of analytics e.g., leads to higher resource consumption, impacting the CPU, and bandwidth, and potentially increasing costs. 

To achieve this, we propose an RL-based predictor component integrated within the orchestrator. This RL-based predictor enables dynamic and autonomous resource allocation, ensuring that the system can meet the specific data analytics requirements (e.g., freshness, coverage, sample size, response time) while considering cost and resource constraints. However, if the architecture cannot provide the necessary resources, the orchestrator can also modify the initial data analytics requirements within predefined boundaries.

%This proposal allows the orchestrator to make intelligent decisions in real-time, improving both resource efficiency and the overall performance of data analytics.

\begin{figure*}[ht]
\centering
\includegraphics[width=\textwidth]{figures/architectureV2.png}
\caption{Multidimensional Elasticity Management in CC}\label{fig:elasticityDimensions}
\end{figure*}

%coste medioambiental/energético’ 

\subsection{Data Analytic Requirements}
Data analytics requirements define the key parameters for executing analytics tasks and are dynamically managed by the orchestrator as part of the elasticity framework. These requirements are defined within certain limits, allowing the orchestrator to modify them as necessary to optimize the balance between system performance and resource availability. The core data analytics requirements managed by the orchestrator include:


\begin{itemize}
    \item Freshness: Indicates the frequency at which the analytics are to be executed. Depending on the purpose of the analytics, it may be necessary to execute them more or less frequently within a given period. %Freshness is represented by the number of executions within a time interval, which can be defined in hours (h), minutes (m), or seconds (s). For example, 34 e/s or 1 e/h.
    
    \item Coverage: Indicates the available locations from which analytical data is desired. It can be specified using identifiers provided by the orchestrator, which are associated with different locations in the infrastructure.
    
    \item Sample: This requirement indicates the percentage of representative samples desired from the specified locations. Within each location, various devices are generating the required information. Depending on the analytics' objective, a complete representative sample or only a portion can be chosen using this parameter.
    
    \item Response Time: Sets the response time desired for delivering the requested analytics. %The maximum response time can be expressed in minutes (m), seconds (s), or milliseconds (ms). For example, 34 ms or 2 s.
   
    \item Cost: Represent the budget desired willing to pay for the execution of the analytics. %The cost is defined in terms of cost per hour (€/h), following conventional SaaS "pay-as-you-go" models, as the analytics will be executed for the required duration.

\end{itemize}

Finally, Figure \ref{fig:elasticityDimensions}b shows the graphical impact of the coverage, freshness, and sample requirements. Expanding the coverage area increases the number of nodes involved in the analysis while increasing freshness requires more frequent updates and data processing. Similarly, a larger sample size means more data needs to be processed and transferred.



% \begin{figure}[ht]
% \centering
% \includegraphics[width=.7\textwidth]{figures/Variables.png}
% \caption{Explanation of Coverage, Freshness and Sample.}\label{fig:variables}
% \end{figure}



\subsection{Architecture Dimensions}

%This section outlines the dimensions monitored and managed within the CC infrastructure. 
Dimensions are grouped into three categories based on the different entities in the architecture: computing nodes, networks, and data. Each category encapsulates critical dimensions that the orchestrator considers when adapting the system to meet analytics requirements and maintain performance.


\begin{itemize}
    \item Computing node: Represents the hardware responsible for executing data analytics within the infrastructure. Key metrics monitored include \textit{CPU} usage, which tracks processing capacity, available RAM (\textit{MEM}), geographical \textit{location}, which identifies where the node is situated, \textit{energy consumption}, referring to the power usage, and \textit{computing cost}, indicating the expense associated with utilizing the node's computational resources.

        % \begin{itemize}
        %     \item CPU: Represents the percentage of CPU usage.
        %     \item MEM: Signifies the amount of available RAM.%, expressed in gigabytes (GB).
        %     \item Location: Identifies the geographical position of the computing node.% through an alphanumeric identifier.
        %     \item Energy Consumption: Reflects the energy consumption of the computing node.%measured in kilowatt-hours (kWh).
        %     \item Computing Cost: Indicates the cost per hour of computational usage on the node.% expressed in euros per hour (€/h).
        % \end{itemize}

    \item Network: The network entity encompasses various aspects related to data transfer and communication between computing nodes. Key metrics include \textit{bandwidth}, which refers to the available capacity for data transfer, \textit{transfer cost}, which is the expense associated with moving data across the network, and \textit{latency}, which measures the time taken to transfer data between nodes.
        % \begin{itemize}
        %     \item Bandwidth: Represents the available bandwidth capacity in the network connection. %measured in megabits per second (Mbps) or gigabits per second (Gbps).
        %     \item Transfer Cost: Cost associated with data transfer, determined based on the volume of data transferred.% and expressed in euros per gigabyte (€/GB). 
        %     \item Latency: Time taking to transfer data between computing nodes.
        % \end{itemize}
    \item Data: The data entity focuses on the properties of the data being processed within the infrastructure. Key metrics include \textit{volume}, which denotes the total amount of data, providing insight into the scale of data processed for resource optimization. \textit{Refresh rate} refers to the frequency at which data is updated from its source, indicating how often new data is available. \textit{Processing time} measures the duration between the start of data analytics and the retrieval of results. Lastly, storage cost reflects the expense associated with storing data in the infrastructure.
        % \begin{itemize}
        %     \item Volume: The volume dimension denotes the total amount of data. 
        %     This metric provides crucial insights into the scale and scope of data being processed, facilitating resource allocation and optimization strategies.
            
        %     \item Refresh rate: The refresh rate dimension represents the frequency at which data is updated from its source, delineating the interval between successive data updates. 
            
        %     \item Processing time: The processing time dimension means the duration elapsed from the initiation of an analytical process to the retrieval of results. 
            
        %     \item Storage cost: The storage cost dimension indicates the expenditure associated with data storage. 
        % \end{itemize}

        
\end{itemize}

\subsection{Relationships Between Data Analytics Requirements and Architecture Dimensions}

%This section explores the relationships and impacts that data analytics requirements have on various dimensions of the infrastructure, highlighting both direct and indirect connections. 
Understanding the relationships and impacts that data analytics requirements have on various dimensions of the infrastructure is critical to managing the performance, resource allocation, and overall efficiency of the CC architecture.

\textbf{Direct relation}: Direct relationships refer to clear, explicit connections between specific data analytics requirements and architecture dimensions. These relationships show how a change in one element directly influences the behaviour or performance of another.

\begin{itemize}
    \item \textit{Coverage and Location:} Coverage determines the geographical locations from which data analytics are conducted, creating a direct link with the Location of computing nodes. A broader coverage area requires more geographically dispersed computing nodes to collect and process data from a larger set of locations.
    
    \item \textit{Sample and Volume:} The Sample size refers to the percentage of data or devices used for data analytics. A larger sample size results in more end devices or data points contributing to the analysis, which in turn increases the total volume of data to be processed and stored.
    
    \item \textit{Freshness and Refresh rate:} Freshness measures how up-to-date the data is, and it is directly tied to the refresh rate of data updates. A higher refresh rate ensures more frequent updates, thereby maintaining the real-time relevance and freshness of the data being analyzed.

    % \item \textit{Response time and Quality parameters:} Response time is the maximum acceptable delay for analytics results, while the quality dimension of the architecture refers to the time elapsed between initiating an analysis and retrieving the results. This includes both processing time and latency. The response time requirement directly correlates with the system's ability to deliver analytics results within the desired timeframe, thus impacting the overall quality of service
    
    
\end{itemize}

\textbf{Indirect relations:} Indirect relationships are more complex and less apparent connections between data analytics requirements and infrastructure dimensions, but they can significantly impact system performance. This work focuses specifically on the impact of coverage, sample, and freshness for CPU due to space limitations. Larger coverage means processing data from more computing nodes, which indirectly increases CPU usage. A larger sample size also adds to the data processing demand, which can increase the CPU usage for processing. Lastly, higher freshness involves more frequent data updates to process, which places a greater load on CPU resources. These indirect effects on CPU usage are critical in shaping overall system performance, as highlighted in Section~\ref{Sec:validation}.

%\begin{itemize}

    %\item Coverage
    %\item \textit{Coverage and Bandwidth:} Expanded coverage can increase data traffic, putting pressure on available bandwidth. This may require a review of network capacity to ensure it can handle the additional load without affecting performance or service quality.

    % \item \textit{Coverage and Energy Consumption:} Broader coverage could also lead to higher energy consumption. With more computing nodes spread across various locations, energy demands increase as more devices are actively transmitting and processing data. 
    
    %\item \textit{Sample and Response time:} A larger sample size increases data processing demands, potentially extending the time required to complete the data analysis and indirectly affecting the system’s ability to meet response time requirements.

    % \item \textit{Sample and Bandwidth:} A larger sample size requires more data to be transferred across the network for analysis, increasing the load on the network’s bandwidth. This could lead to congestion, reduced network performance, and, consequently, longer response times for analytics tasks.


    % \item \textit{Freshness and Energy consumption:} Increased freshness—achieved through more frequent data updates—places a heavier workload on the processing nodes. This greater processing demand, in turn, increases the energy consumption of the nodes, as they must work harder and more frequently to keep the data up-to-date.
    
    %\item \textit{Freshness and CPU:} Higher freshness levels increase the workload on computing nodes, leading to increased CPU. Enhanced freshness requires additional processing power and CPU resources, placing more strain on the infrastructure.

    % \item \textit{Freshness and Volume:} A higher freshness can indirectly increase the total volume of data over time. Frequent updates generate more data within a given period, leading to a cumulative increase in the amount of data that must be stored and processed.
    
%\end{itemize}

%These relationships guide the orchestration process, enabling dynamic adjustments to ensure that the system remains efficient while balancing resource constraints and performance demands.


\subsection{Orchestrator}


The orchestrator is a pivotal component in the CC architecture, responsible for managing the elastic requirements of data analytics, and adapting the infrastructure to the evolving needs of both the architecture and the analytics. By continuously monitoring the state of the infrastructure and analytics requirements, the orchestrator ensures that resources are allocated efficiently to meet the performance goals set by the system. However, when the available resources are insufficient to meet the specified analytics requirements, the orchestrator is also capable of adjusting the initial data analytics requirements to ensure that the system continues to function optimally under resource constraints. This dynamic adaptation of both the infrastructure and analytics requirements ensures a balance between performance, cost, and resource availability.

The orchestrator uses an RL-based predictor to dynamically adjust resources in real-time, making it capable of autonomously optimizing the infrastructure based on analytics demands and resource availability. If the infrastructure cannot be sufficiently adapted to meet the data analytics requirements, the orchestrator will modify those requirements. The orchestrator consists of three main modules that work in tandem, as illustrated in Fig.~\ref{fig:orchestrator}, which are detailed below:



    \subsubsection{Architecture Monitor} This module is responsible for continuously tracking the resource dimensions of the architecture. It gathers metrics related to available resources such as CPU usage, memory, network bandwidth, or energy consumption. Additionally, it monitors costs and other critical data points, such as response time and service-level performance, ensuring that the orchestrator has a real-time snapshot of the system's operational status. %If the infrastructure cannot be adjusted to meet the analytics requirements, the orchestrator may reduce the expectations of certain requirements, such as data freshness or response time, to ensure the system operates within the current resource limitations.

    \subsubsection {Analytics Monitor} The Analytics Monitor oversees the status of the data analytics running on the system. This module collects and stores the requirements that consumers specify, such as data freshness, coverage, and sample size. These requirements are then compared with the real-time status of the system, as reported by the Architecture Monitor, to identify potential mismatches or inefficiencies. If the system's resources cannot meet these requirements, the orchestrator will adjust the analytics requirements within predefined limits to maintain system stability and performance.

    \subsubsection{RL-based Predictor} This module is responsible for comparing the actual infrastructure information from the Architecture Monitor and the analytics requirements of the Analytics Monitor. Its purpose is to adapt the infrastructure to meet the data analytics requirements as much as possible within the limits of the infrastructure resources. In this setup, the RL agent aims to optimize the orchestration by learning which actions (e.g., increasing CPU resources, adjusting network bandwidth, etc.) yield the best performance while considering the elastic dimensions: quality, resource availability, and cost. More specifically, the RL-based predictor is modeled as an agent that interacts with the CC (i.e., the environment) to learn an optimal policy for resource allocation. The RL-based predictor adjusts infrastructure resources to meet analytics requirements and contains the following key elements:

        \begin{itemize}
            \item \textbf{State (S)} includes the current infrastructure metrics (e.g., CPU usage, memory availability, network bandwidth, and energy consumption) and the analytics requirements (e.g., coverage, freshness, sample size, response time). 
           %next paper  
           %\[
            %   S_t = \{ \text{CPU}_t, \text{M}_t, \text{BW}_t, \text{EC}_t, \text{V}_t, \text{RR}_t, \text{RT}_t, \text{C}_t \}
           %\]
            
             
            \item \textbf{Action (A)} involves adjusting resource allocations, such as increasing or decreasing device resource usage (e.g., CPU or memory), network usage (i.e., modifying bandwidth), or changing the frequency of analytics executions (freshness), etc. These actions modify the current state aiming to optimize infrastructure resources and meet analytics requirements.
        %next paperr
          %  \[
           %    A_t = \{ \text{CPU}_t, \text{M}_t,  \text{BW}_t,  \text{EC}_t, \text{F}_t, \text{SM}_t \}
           % \]
         %   where $\text{CPU}_t$ represents a change in CPU allocation (increase or decrease) at time $t$, and so on.
            
            \item \textbf{Reward (R)} is a scalar value that represents the system performance after an action is taken. We reward positive actions that successfully execute analytics within cost limits. Negative rewards are given for actions that do not meet requirements, overuse resources, or exceed costs. %Therefore, the reward function is designed as in the following:
        %next paper
        %    \[
        %    R_t = w_1 \cdot \text{Q}_t + w_2 \cdot (C_{\max} - C_t) - w_3 \cdot \text{RT}_t
        %   \]

        %   where $Q_t$ represents quality of analytics, $C_{max}$ represents maximum allowed cost, $C_t$ represents current resource cost, $RT_t$ represents current response time, and lastly $w_1, w_2, w_3$ represent weight factors for quality, cost, and response time.
            
            \item \textbf{Policy (P)} is the strategy used by the RL agent to decide which action to execute based on the current state. Specifically, the RL agent's goal is to find an optimal that maximizes the expected reward. The RL agent iteratively updates its policy to improve overall decisions (i.e., through exploration and exploitation). %(i.e., trying new actions)$ (i.e., using actions known to perform well)). %The RL agent learns this policy through system interaction, receiving rewards reflecting how well actions meet goals (e.g., cost savings or improved analytics).

           %next paper
        %   \[
          %  P^* = \arg\max_{A_t} Q^*(S_t, A_t)
          %  \]
         
       %  $Q^*(S_t, A_t)$ represents the optimal Q-function which gives the cumulative reward when executing action $A_t$ in state $S_t$. Nevertheless, 
      % The RL agent iteratively updates its policy to improve overall decisions (i.e.,  refining its policy through exploration (i.e., trying new actions) and exploitation (i.e., using actions known to perform well)). The RL agent learns this policy through system interaction, receiving rewards reflecting how well actions meet goals (e.g., cost savings or improved analytics).
        \end{itemize}




    % \subsubsection{Action} %The adapt component is in charge of receiving the changes proposed by the Evaluator component and carrying those changes into the infrastructure. To do so, the component manages the current state of the analytics requirements and sends the necessary instructions to execute the proposed changes. \textcolor{red}{Todo...}


\begin{figure}[ht]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/orchestrator.png}
    \caption{Orchestrator with RL-Based Elasticity Management in the CC.}\label{fig:orchestrator}
\end{figure}

%It is important to note that the analytics requirements on which the orchestrator acts directly are Freshness, Coverage, and Sample. These requirements are modified within the range of values carefully set by consumers to adjust the data update frequency, the location from which analytics will be performed, and the size of the representative sample used in the analysis, respectively. These are the parameters that can be directly modified to optimize the performance of the analytics according to the specific needs of the users. However, there is a significant exception with the response time requirement and cost. These requirements cannot be directly modified in the infrastructure, as their value results from the complex interaction between the other dimensions.





\subsection{Case study \& Workflow}

%To demonstrate the functionality of the proposed infrastructure, a case study is presented involving a multinational electronic components manufacturer. The company operates multiple manufacturing facilities worldwide and aims to improve production efficiency through advanced data analysis to identify risks, optimizations, and process improvements.

To demonstrate the functionality of the proposed infrastructure, a case study is presented involving a smart city deployment, where the city aims to improve urban planning and public safety through advanced data analytics. The system monitors human movement in different areas of the city to generate heatmaps that help identify patterns, risks, and opportunities for optimizing city services.

%The company has implemented a distributed infrastructure with nodes equipped to process and store data analytics. An advanced orchestrator coordinates the execution of analytics, ensuring that the specified requirements are met. The infrastructure is hierarchical, with a central main or head node aggregating data from edge nodes located at each factory. These edge nodes collect information from local sensors.

The city has implemented a distributed infrastructure with nodes equipped to process and store data analytics. The orchestrator coordinates the execution of data analytics, ensuring that the specified data analytics requirements are met. The infrastructure is hierarchical, with a central head node aggregating data from edge nodes located across different parts of the city. These edge nodes collect information from local sensors monitoring a person's movement. The following is a description of how the system would work.

\begin{enumerate}
    \item \textit{Architecture and Analytics requirements Gathering:} The orchestrator collects data on infrastructure resources and data analytics requirements to inform decision-making.
    
    \item \textit{Predictor Evaluation:} The predictor evaluates the current state of infrastructure and analytics needs to determine whether resource or analytics adjustments are required.

    \item \textit{State Changes and Adaptation:} Based on the predictor’s analysis, the orchestrator decides whether to adjustparameters (e.g., reducing coverage or sample size) or reallocate resources to maintain system performance.

    \item \textit{Action:} The orchestrator dynamically allocates resources or/and modulates analytics requirements to ensure efficient execution while balancing resource usage.

    \item \textit{Continous Monitoring and Adaptation:} The orchestrator continuously monitors system performance in real-time, adjusting based on feedback to optimize data quality and processing time.
\end{enumerate}

==> __4.Validation.tex.v0 <==

% \section{Emerging Agenda} \label{Sec:validation}

% Elasticity in the CC architecture plays a crucial role in enabling both infrastructure and application requirements to adapt dynamically to evolving conditions. However, integrating learning techniques in the orchestrator, which operates in dynamic environments, presents several challenges. We highlight four key research directions that require further exploration in the future:

% %Reinforcement learning agent

% \begin{itemize}


% \item Trustworthiness: Learning models become more integrated into cloud orchestration; therefore, ensuring the transparency, explainability, and trustworthiness of these models becomes essential. Specifically, future research should explore methods for making decision processes in learning-based orchestrators more interpretable (i.e., enabling operators to understand and trust the system’s actions).

% \item LLM-based Data Analytic Requirements: Large Models must become more integrated into cloud orchestration. This means that we will need to realize a natural language interface for the data stakeholders to "talk to the continuum about their data requirements". Therefore, future research should explore methods such as neural symbolic AI, chatbots, LLM, and generative AI.


%     \item Novel proposal for Continuum architectures
%     \item Research challenges:
%     \begin{itemize}
%         \item Scalability in Continuum architecture: management of multiples nodes and requirements
%         \item Multi-agent for manage differents parts of the Continuum?
%         \item Use of LSTM techniques
%         \item Rapidly adaptation to changes
%     \end{itemize}
% \end{itemize}
 
% LLM for define data analytics requirements and the limits? Or only for future works



\section{Evaluation and impact of data analytics requirements} \label{Sec:validation}

This section evaluates the impact of data analytics requirements (i.e., coverage, sample, and freshness) on CPU usage across the infrastructure. The infrastructure consists of a \textit{headnode} and three edge nodes (\textit{edgenode1}, \textit{edgenode2}, \textit{edgenode3}), simulating a system that generates heatmaps of the city’s different areas using the One simulator to generate the person movement dataset~\cite{jesus2021oppnets}. The edge nodes generate a heatmap of their respective areas, which are then aggregated by the head node to produce a unified heatmap. The results are shown in Fig.~\ref{fig:dataAnalyticsImpact}, with three subfigures (a), (b), and (c), corresponding to the impact of increasing coverage, sample, and freshness respectively.


\begin{figure*}[htpb]
\centering
\includegraphics[width=\textwidth]{figures/validation/analyticsReqValidation.png}
\caption{Impact of analytics requirements on CPU usage.}\label{fig:dataAnalyticsImpact}
\end{figure*}

In Fig.~\ref{fig:dataAnalyticsImpact}a, we observe that as coverage increases, more edge nodes are progressively engaged, leading to a staggered rise in CPU usage. Initially, only one \textit{edgenode} is active, but as more geographic areas are covered, additional nodes become involved, creating a stepwise pattern in CPU utilization. Simultaneously, the \textit{headnode's} CPU usage also rises as it processes the increasing amount of data from multiple edge nodes. In Fig.~\ref{fig:dataAnalyticsImpact}b, as the sample increases, CPU usage gradually rises across all edge nodes. Similarly, the \textit{headnode} shows a CPU increase as it processes the increasing volume of data. This behavior reflects how larger samples translate to the collection of more data for analytics, resulting in higher processing demands for both the edge nodes and the \textit{headnode}, which aggregates all the incoming data. In Fig.~\ref{fig:dataAnalyticsImpact}c, as freshness increases, there is a higher demand for frequent data updates. The edge nodes show a relatively constant CPU usage but with an increased periodicity of spikes as freshness increases. This indicates that the system is processing updates more frequently. However, the \textit{headnode} exhibits a more gradual increase in CPU usage, reflecting the higher frequency of data processing as it aggregates information from the three edge nodes at an increased rate. In summary, the assessment highlights the significant impact of these data analytics requirements on the entire CC infrastructure. These results underscore the importance of multi-dimensional elasticity and the ability of the orchestrator to dynamically adjust these analytics requirements. When infrastructure resources cannot be scaled or optimized, the orchestrator can adapt these requirements to maintain system performance, ensuring a flexible and balanced response to fluctuations in workloads and resource availability.


%Details
% Actions: When the CPU usage is near to 100%, it modifies sample, if CPU not decrease, it modifies freshness (for all analytics).

Finally, an experiment is shown that demonstrates the operation of the orchestrator developed on the basis of the MDP. %Fig.~\ref{fig:orchestration-analytics} shows an extract of an initial version of the orchestrator based on the Markov Decision Process (MDP). 
In this experiment, a heuristic is used to manage fixed values for transitions and actions, effectively serving as a policy for the MDP. The orchestrator monitors CPU utilization across all infrastructure and adjusts the data analytics requirements dynamically to prevent overloading any of the nodes. The system adjusts based on CPU usage to optimize resource allocation in real-time.

In this setup, the heuristic policy dictates the architecture’s actions according to the current state of CPU usage. 
When the CPU usage is low, the orchestrator takes the action NO-OP (no operation), leaving the data analytics requirements unchanged. However, when CPU usage approaches 100\%, the orchestrator transitions to a new state where it adjusts the data analytics by modifying the sample size and reducing the data processed to ease the CPU usage. If high CPU usage persists after this, the orchestrator modifies the freshness, reducing the frequency of data updates to alleviate resources. If it persists, as a last resort, decrease the coverage, eliminating the execution of data analytics on different nodes. This sequence of state transitions and actions allows the orchestrator to systematically balance the workload across the system, ensuring that resources are used efficiently and avoiding overutilization. As seen in Fig.~\ref{fig:orchestration-analytics}, it can be observed how CPU shows an increase, prompting the orchestrator to first adjust the sample size to reduce the load. As high usage persists, the orchestrator then modifies the freshness, decreasing update frequency and relieving CPU usage to maintain system balance.

%is managed by dynamically adjusting the data analysis requirements. The orchestrator monitors CPU utilization across all infrastructure, ensuring that none of the nodes are overloaded. By modulating the data analytics requirements, the orchestrator optimizes resource allocation in real-time. As seen in the graph, the CPU usage fluctuates as the orchestrator adapts these parameters based on current resource availability, ensuring that CPU usage remains balanced and preventing overutilization.




\begin{figure}[ht]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/validation/orchestration.png}
    \caption{Orchestrator adapting data analytics requirements to manage CPU usage.}\label{fig:orchestration-analytics}
    %Adaptative Data Analytics Management for CPU Usage
\end{figure}






==> architecture_copy.tex <==
\section{Adaptive Elasticity for Data Analytics in the Cloud Continuum} \label{Sec:architecture}



% The general dimensions of elasticity are subdivided into specific dimensions, which can be defined from two perspectives, at the operational level and at the application level as shown in Figure \ref{fig:elasticityDimensions}:
% \begin{itemize}
%     \item Computing Node Elasticity (operational level): refers to the dimensions that allow for adaptability of the computing nodes implemented in the infrastructure. The general dimensions covered are resources (to adjust CPU, memory, or energy consumption) and cost (to adjust the cost per use).
%     \item Analytic Elasticity (application level): refers to the dimensions that allow adapting the needs of the analytics proposed by the consumers. The general dimensions covered are quality (to adjust expected quality, expected response time, or frequency of the data) and cost (how much is willing to pay).
% \end{itemize}

%---------------%

Elasticity within the Cloud Continuum architecture is a key factor in ensuring that both infrastructure and application requirements can dynamically adjust to changing conditions. This elasticity is distributed across multidimensional that span two major levels: operational and application. These dimensions, illustrated in Figure\ref{fig:elasticityDimensions}, reflect the different factors that influence the adaptability of both computing resources and the data analytics themselves.


Elasticity within the Cloud Continuum architecture is fundamental to enabling the dynamic adaptation of both infrastructure resources and data analytics requirements. This elasticity spans multiple dimensions that impact both the operational efficiency and the performance of analytics applications. In this context, we propose a comprehensive framework for managing multi-dimensional elasticity in data analytics for the Cloud Continuum. These dimensions, illustrated in Figure\ref{fig:elasticityDimensions}, reflect the different factors that influence the adaptability of both computing resources and the data analytics themselves.


At the operational level, elasticity focuses on the efficient use of resources like CPU, memory, and energy, ensuring that these computing resources can adjust dynamically to changing workloads. This level also involves managing the cost associated with using infrastructure resources, particularly in environments where resource consumption is billed based on usage.

At the application level, elasticity manages the specific requirements of data analytics, such as the quality of results, the frequency at which data is processed, and the timeliness of the analytics outcomes. These dimensions require careful balancing by the orchestrator to ensure that the infrastructure can meet the performance expectations without exceeding resource or cost limitations.

These dimensions are interrelated, as changes in one can affect others. For instance, increasing the sample size to improve the quality of analytics will lead to higher resource consumption, impacting the CPU, and bandwidth, and potentially increasing costs. 

To achieve this, we propose a novel Reinforcement Learning (RL) predictor component integrated within the orchestrator. This RL-based predictor enables dynamic and autonomous resource allocation, ensuring that the system can meet the specific data analytics requirements (e.g., freshness, coverage, sample size, response time) while considering cost and resource constraints. However, if the architecture cannot provide the necessary resources, the orchestrator also can modify the initial data analytics requirements within predefined boundaries.

%This proposal allows the orchestrator to make intelligent decisions in real-time, improving both resource efficiency and the overall performance of data analytics.

\begin{figure*}[ht]
\centering
\includegraphics[width=0.7\textwidth]{figures/architectureV2.png}
\caption{Multidimensional Elasticity Management in Cloud Continuum: Relationships Between Data Analytics Requirements and Architecture Dimensions.}\label{fig:elasticityDimensions}
\end{figure*}

%coste medioambiental/energético’ 

\subsection{Data Analytic Requirements}
Data analytics requirements define the key parameters for executing analytics tasks, and they are dynamically managed by the orchestrator as part of the elasticity framework. These requirements are defined within certain limits, allowing the orchestrator to modify them as necessary to optimize the balance between system performance and resource availability. The core data analytics requirements managed by the orchestrator include:


\begin{itemize}
    \item Freshness: Indicates the frequency at which the analytics are to be executed. Depending on the purpose of the analytics, it may be necessary to execute them more or less frequently within a given period. %Freshness is represented by the number of executions within a time interval, which can be defined in hours (h), minutes (m), or seconds (s). For example, 34 e/s or 1 e/h.
    
    \item Coverage: Indicates the available locations from which analytical data is desired. It can be specified using identifiers provided by the orchestrator, which are associated with different locations in the infrastructure.
    
    \item Sample: This requirement indicates the percentage of representative samples desired from the specified locations. Within each location, various devices are generating the required information. Depending on the analytics' objective, a complete representative sample or only a portion can be chosen using this parameter.
    
    \item Response Time: Sets the response time desired for delivering the requested analytics. %The maximum response time can be expressed in minutes (m), seconds (s), or milliseconds (ms). For example, 34 ms or 2 s.
   
    \item Cost: Represent the budget desired is willing to pay for the execution of the analytics. %The cost is defined in terms of cost per hour (€/h), following conventional SaaS "pay-as-you-go" models, as the analytics will be executed for the required duration.

\end{itemize}

Finally, Figure \ref{fig:variables} shows the graphical impact of the Coverage, Freshness, and Sample requirements. Expanding the coverage area increases the number of nodes involved in the analysis, while increasing freshness requires more frequent updates and data processing. Similarly, a larger sample size means more data needs to be processed and transferred.



\begin{figure}[ht]
\centering
\includegraphics[width=.5\textwidth]{figures/Variables.png}
\caption{Explanation of Coverage, Freshness and Sample.}\label{fig:variables}
\end{figure}



\subsection{Architecture Dimensions}

This section outlines the dimensions monitored and managed within the Cloud Continuum infrastructure. These variables are grouped into three categories based on the different entities in the architecture: computing nodes, the network, and the data. Each category encapsulates critical dimensions that the orchestrator considers when adapting the system to meet analytics requirements and maintain performance.


\begin{itemize}
    \item Computing node: Represents the hardware components of the infrastructure responsible for executing the data analytics.
        \begin{itemize}
            \item CPU: Represents the percentage of CPU usage.
            \item MEM: Signifies the amount of available RAM.%, expressed in gigabytes (GB).
            \item Location: Identifies the geographical position of the computing node.% through an alphanumeric identifier.
            \item Energy Consumption: Reflects the energy consumption of the computing node.%measured in kilowatt-hours (kWh).
            \item Computing Cost: Indicates the cost per hour of computational usage on the node.% expressed in euros per hour (€/h).
        \end{itemize}

    \item Network: The network entity includes various aspects related to the data transfer and communication between the computing nodes.
        \begin{itemize}
            \item Bandwidth: Represents the available bandwidth capacity in the network connection. %measured in megabits per second (Mbps) or gigabits per second (Gbps).
            \item Transfer Cost: Cost associated with data transfer, determined based on the volume of data transferred.% and expressed in euros per gigabyte (€/GB). 
            \item Latency: Time taking to transfer data between computing nodes.
        \end{itemize}
    \item Data: The data entity focuses on the properties and characteristics of the data being processed within the infrastructure.
        \begin{itemize}
            \item Volume: The volume dimension denotes the total amount of data. %quantified in megabytes (MB), kilobytes (KB), or gigabytes (GB). 
            This metric provides crucial insights into the scale and scope of data being processed, facilitating resource allocation and optimization strategies.
            
            \item Refresh rate: The refresh rate dimension represents the frequency at which data is updated from its source, delineating the interval between successive data updates. %Expressed as the number of updates within a defined time period, typically in hours (h), minutes (m), or seconds (s), this metric elucidates the timeliness and currency of the data being utilized. For instance, a refresh rate of "34 u/s" means 34 updates per second, or "1 u/h" indicates one update per hour.
            
            \item Processing time: The processing time dimension means the duration elapsed from the initiation of an analytical process to the retrieval of results. %Measured in minutes (m), seconds (s), or milliseconds (ms).
            
            \item Storage cost: The storage cost dimension indicates the expenditure associated with data storage. %expressed in euros per gigabyte (€/GB).
        \end{itemize}

        
\end{itemize}

\subsection{Relationships Between Data Analytics Requirements and Architecture Dimensions}

This section explores the relationships and impacts that data analytics requirements have on various dimensions of the infrastructure, highlighting both direct and indirect connections. Understanding these relationships is critical to managing the performance, resource allocation, and overall efficiency of the cloud continuum architecture.

\textbf{Direct relation}: Direct relationships refer to clear, explicit connections between specific data analytics requirements and architecture dimensions. These relationships show how a change in one element directly influences the behaviour or performance of another.

\begin{itemize}
    \item \textit{Coverage and Location:} Coverage determines the geographical locations from which data analytics are conducted, creating a direct link with the Location of computing nodes. A broader coverage area requires more geographically dispersed computing nodes to collect and process data from a larger set of locations.
    
    \item \textit{Sample and Volume:} The Sample size refers to the percentage of data or devices used for data analytics. A larger sample size results in more end devices or data points contributing to the analysis, which in turn increases the total volume of data to be processed and stored.
    
    \item \textit{Freshness and Refresh rate:} %The data update frequency, represented by the refresh rate, is directly related to the freshness of the data. A higher refresh rate implies a more frequent data update, contributing to keeping the data updated and relevant in real-time. This, in turn, translates to greater freshness of the data available for analysis.
    Freshness measures how up-to-date the data is, and it is directly tied to the refresh rate of data updates. A higher refresh rate ensures more frequent updates, thereby maintaining the real-time relevance and freshness of the data being analyzed.

    \item \textit{Response time and Quality parameters:} Response time is the maximum acceptable delay for analytics results, while the quality dimension of the architecture refers to the time elapsed between initiating an analysis and retrieving the results. This includes both processing time and latency. The response time requirement directly correlates with the system's ability to deliver analytics results within the desired timeframe, thus impacting the overall quality of service
    
    
\end{itemize}

\textbf{Indirect relations:} Indirect relationships are more complex and less obvious connections between analytics requirements and infrastructure dimensions. These relationships may not be immediately apparent but can have a significant impact on system performance. The following are some of the existing ones.

\begin{itemize}

    % Coverage: cost (computing and transfer), energy consumption, CPU, mem, bandwidth, response time

    % Sample: cost (computing and transfer), energy consumption, CPU, mem, bandwidth, response time

    % Freshness: cost (computing and transfer), energy consumption, CPU, mem, bandwidth, response time (latency and processing time)

    %\item Coverage
    \item \textit{Coverage and Bandwidth:} Expanded coverage of analytics may lead to increased data traffic across the network, potentially exerting pressure on the available bandwidth. This might necessitate a review of the network's capacity to ensure it can handle the surge in data flow without compromising performance or service quality.

    \item \textit{Coverage and Energy Consumption:} Broader coverage could also lead to higher energy consumption. With more computing nodes spread across various locations, energy demands increase as more devices are actively transmitting and processing data. 
    
    \item \textit{Sample and Response time:} A larger sample size may result in increased data processing demands, which could prolong the time required to complete the analysis. This highlights an indirect relationship where larger samples can negatively impact the system’s ability to meet response time requirements.

    \item \textit{Sample and Bandwidth:} A larger sample size requires more data to be transferred across the network for analysis, increasing the load on the network’s bandwidth. This could lead to congestion, reduced network performance, and, consequently, longer response times for analytics tasks.


    \item \textit{Freshness and Energy consumption:} Increased freshness—achieved through more frequent data updates—places a heavier workload on the processing nodes. This greater processing demand, in turn, increases the energy consumption of the nodes, as they must work harder and more frequently to keep the data up-to-date.
    
    \item \textit{Freshness, CPU, and MEM:} Higher freshness levels could escalate the workload on computing nodes, affecting CPU and MEM usage. Enhanced data freshness may require additional processing and memory resources to handle the increased workload. Consequently, computing nodes may experience an uptick in CPU and MEM usage.

    \item \textit{Freshness and Volume:} A higher freshness can indirectly increase the total volume of data over time. Frequent updates generate more data within a given period, leading to a cumulative increase in the amount of data that must be stored and processed.
    
\end{itemize}

%These relationships guide the orchestration process, enabling dynamic adjustments to ensure that the system remains efficient while balancing resource constraints and performance demands.


\subsection{Orchestrator}


The orchestrator is a pivotal component in the Cloud Continuum architecture, responsible for managing the elastic requirements of data analytics, and adapting the infrastructure to the evolving needs of both the architecture and the analytics. By continuously monitoring the state of the infrastructure and analytics requirements, the orchestrator ensures that resources are allocated efficiently to meet the performance goals set by the system. However, when the available resources are insufficient to meet the specified analytics requirements, the orchestrator is also capable of adjusting the initial data analytics requirements to ensure that the system continues to function optimally under resource constraints. This dynamic adaptation of both the infrastructure and analytics requirements ensures a balance between performance, cost, and resource availability.

The orchestrator uses a Reinforcement Learning (RL)-based predictor to dynamically adjust resources in real-time, making it capable of autonomously optimizing the infrastructure based on analytics demands and resource availability. If the infrastructure cannot be sufficiently adapted to meet the data analytics requirements, the orchestrator will modify those requirements. The orchestrator consists of three main modules that work in tandem, as illustrated in Figure ~\ref{fig:orchestrator}, which are detailed below:



    \subsubsection{Architecture Monitor} This module is responsible for continuously tracking the resource dimensions of the architecture. It gathers metrics related to available resources such as CPU usage, memory, network bandwidth, or energy consumption. Additionally, it monitors costs and other critical data points, such as response time and service-level performance, ensuring that the orchestrator has a real-time snapshot of the system's operational status. %If the infrastructure cannot be adjusted to meet the analytics requirements, the orchestrator may reduce the expectations of certain requirements, such as data freshness or response time, to ensure the system operates within the current resource limitations.

    \subsubsection {Analytics Monitor} The Analytics Monitor oversees the status of the data analytics running on the system. This module collects and stores the requirements that consumers specify, such as data freshness, coverage, and sample size. These requirements are then compared with the real-time status of the system, as reported by the Architecture Monitor, to identify potential mismatches or inefficiencies. If the system's resources cannot be adjusted to meet these requirements, the orchestrator will modify the analytics requirements—within predefined boundaries—such as lowering the sample size or reducing the frequency of data updates, to maintain system stability and performance.

    \subsubsection{RL-based Predictor} This module is in charge of comparing the actual infrastructure information from the Architecture Monitor and the analytics requirements from the Analytics Monitor. Its purpose is to adapt the infrastructure to meet the data analytics requirements as much as possible within the limits of the infrastructure resources. In this setup, the RL agent (predictor) aims to optimize the orchestration by learning which actions (e.g., increasing CPU resources, adjusting network bandwidth, etc.) yield the best performance while considering the elastic dimensions: quality, resource availability, and cost. More specifically, the RL-based predictor is modeled as an agent that interacts with the cloud continuum (i.e., the environment) to learn an optimal policy for resource allocation. The introduced RL-based predictor continuously adapts infrastructure resources in response to analytics requirements. Furthermore, the RL module contains the following key elements:

        \begin{itemize}
            \item \textbf{State (S)} at time $t$ includes the current infrastructure metrics (e.g., CPU usage, memory availability, network bandwidth, and energy consumption) and the analytics requirements (e.g., coverage, freshness, sample size, response time). 
           %next paper  
           %\[
            %   S_t = \{ \text{CPU}_t, \text{M}_t, \text{BW}_t, \text{EC}_t, \text{V}_t, \text{RR}_t, \text{RT}_t, \text{C}_t \}
           %\]
            
             
            \item \textbf{Action (A)} at time $t$ involve adjusting resource allocations, such as increasing or decreasing device resource usage (e.g., CPU or memory), network usage (i.e., modifying bandwidth), or changing the frequency of analytics executions (freshness), etc. These actions modify the current state aiming to optimize infrastructure resources and meet analytics requirements.
        %next paperr
          %  \[
           %    A_t = \{ \text{CPU}_t, \text{M}_t,  \text{BW}_t,  \text{EC}_t, \text{F}_t, \text{SM}_t \}
           % \]
         %   where $\text{CPU}_t$ represents a change in CPU allocation (increase or decrease) at time $t$, and so on.
            
            \item \textbf{Reward (R)} at time $t$ is a scalar value that represents the system performance after an action is taken. 
            We reward positive actions that successfully execute analytics within cost limits. Negative rewards are given for actions that don't meet requirements, overuse resources, or exceed costs. Therefore, the reward function is designed as in the following:
        %next paper
        %    \[
        %    R_t = w_1 \cdot \text{Q}_t + w_2 \cdot (C_{\max} - C_t) - w_3 \cdot \text{RT}_t
        %   \]

        %   where $Q_t$ represents quality of analytics, $C_{max}$ represents maximum allowed cost, $C_t$ represents current resource cost, $RT_t$ represents current response time, and lastly $w_1, w_2, w_3$ represent weight factors for quality, cost, and response time.
            
            \item \textbf{Policy (P)} can be represented as $P(A_t | S_t)$, which is the strategy used by the RL agent to decide which action $A_t$ to execute based on the current state $S_t$. Specifically, the RL agent's goal is to find an optimal $P^*$ that maximizes the expected reward. The RL agent iteratively updates its policy to improve overall decisions (i.e.,  refining its policy through exploration (i.e., trying new actions) and exploitation (i.e., using actions known to perform well)). %The RL agent learns this policy through system interaction, receiving rewards reflecting how well actions meet goals (e.g., cost savings or improved analytics).

           %next paper
        %   \[
          %  P^* = \arg\max_{A_t} Q^*(S_t, A_t)
          %  \]
         
       %  $Q^*(S_t, A_t)$ represents the optimal Q-function which gives the cumulative reward when executing action $A_t$ in state $S_t$. Nevertheless, 
      % The RL agent iteratively updates its policy to improve overall decisions (i.e.,  refining its policy through exploration (i.e., trying new actions) and exploitation (i.e., using actions known to perform well)). The RL agent learns this policy through system interaction, receiving rewards reflecting how well actions meet goals (e.g., cost savings or improved analytics).
        \end{itemize}




    % \subsubsection{Action} %The adapt component is in charge of receiving the changes proposed by the Evaluator component and carrying those changes into the infrastructure. To do so, the component manages the current state of the analytics requirements and sends the necessary instructions to execute the proposed changes. \textcolor{red}{Todo...}


\begin{figure}[ht]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/orchestrator.png}
    \caption{Orchestrator with RL-Based Elasticity Management in the Cloud Continuum.}\label{fig:orchestrator}
\end{figure}

%It is important to note that the analytics requirements on which the orchestrator acts directly are Freshness, Coverage, and Sample. These requirements are modified within the range of values carefully set by consumers to adjust the data update frequency, the location from which analytics will be performed, and the size of the representative sample used in the analysis, respectively. These are the parameters that can be directly modified to optimize the performance of the analytics according to the specific needs of the users. However, there is a significant exception with the response time requirement and cost. These requirements cannot be directly modified in the infrastructure, as their value results from the complex interaction between the other dimensions.

\subsection{Case study \& Workflow}

To demonstrate the functioning of the proposed infrastructure, a case study is described to help the understanding of the proposal.

A multinational company that manufactures electronic components in different facilities around the world. Each facility produces a variety of products and operates its manufacturing infrastructure. To maintain their competitive position in the market, they have set out to improve the efficiency of their production process by using advanced data analytics to identify risks, improvements, and possible optimizations. 

To achieve this, they have deployed a distributed infrastructure that allows them to launch and run data analytics efficiently. Each node is equipped with the processing and storage resources necessary to run these analytics. An advanced orchestrator would monitor and coordinate the execution of these analytics, ensuring that the established requirements are met. In terms of organization, the hierarchy would be composed of a main or root node that would receive the results of the analytics, while in each of the factories, there would be another node in charge of collecting data from the various available sensors.

The following is a description of how the system would work.

\begin{enumerate}
    \item Requirements Gathering: The orchestrator receives data analytics requirements from supervisors or internal management systems. These requirements include the desired geographic coverage (Coverage), data update frequency (Freshness), sample size (Sample), expected response time (Response time) and cost limits (Cost).
    
    \item Availability Evaluation: The orchestrator evaluates the availability of resources, both in terms of processing power, storage, network bandwidth, and any other resources needed to run the analytics. It analyses whether the current infrastructure can meet the requested requirements or whether adjustments or improvements are required.


    \item Resource Planning and Allocation: Once resource requirements and availability have been assessed, the orchestrator plans and allocates the resources needed to run the data analytics efficiently and effectively. It can distribute the analytical tasks among the different processing nodes, adjust the data update frequency, or modify the sample size.

    \item Monitoring: During the execution of analytics, the orchestrator monitors in real time the resources and performance of the infrastructure and the progress of data analytics. It monitors compliance with established requirements, such as response time, data freshness, and costs, and takes corrective action if necessary.

    \item Elasticity: The orchestrator makes adjustments based on changes in resource availability and data analytics requirements. It can reallocate resources, modify analytics settings, or implement new strategies to ensure requirements are met.
\end{enumerate}
